Approximating Bin Packing with Conflict Graphs via Maximization Techniques

We give a comprehensive study of bin packing with conflicts (BPC). The input is a set $I$ of items, sizes $s:I \rightarrow [0,1]$, and a conflict graph $G = (I,E)$. The goal is to find a partition of $I$ into a minimum number of independent sets, each of total size at most $1$. Being a generalization of the notoriously hard graph coloring problem, BPC has been studied mostly on polynomially colorable conflict graphs. An intriguing open question is whether BPC on such graphs admits the same best known approximation guarantees as classic bin packing. We answer this question negatively, by showing that (in contrast to bin packing) there is no asymptotic polynomial-time approximation scheme (APTAS) for BPC already on seemingly easy graph classes, such as bipartite and split graphs. We complement this result with improved approximation guarantees for BPC on several prominent graph classes. Most notably, we derive an asymptotic $1.391$-approximation for bipartite graphs, a $2.445$-approximation for perfect graphs, and a $\left(1+\frac{2}{e}\right)$-approximation for split graphs. To this end, we introduce a generic framework relying on a novel interpretation of BPC allowing us to solve the problem via maximization techniques. Our framework may find use in tackling BPC on other graph classes arising in applications.

==> BP.tex <==


\section{Coloring}
\label{sec:BP}

\begin{lemma}
	\label{lem:coloring}
	Given Bin Packing with some conflict graph $G$, for which there exists an algorithm with $\alpha$- approximation for finding the chromatic number of $G$, we can find a $\alpha+2$ approximation for bin packing with $G$. 
\end{lemma}

\section{Split graph}

Observe the clique $K$ and the independent set $S$. Find a solution with LP. there are at most $m$ fractional items. Each fractional item which is larger than $\frac{1}{2}$, find a packing for it in $k$ (if possible) using maximum matching. Observe the removed items from this matching.

\begin{enumerate}
	\item If there is one evicted item - then because its size is at most half - this is easy. 
	
	\item If there are two and their total size together is at least $\frac{3}{4}$, then the size of the large item is at least $\frac{5}{8}$ otherwise we do not need to evict one of the items. Thus,  the total size of this bin in $\frac{3}{4}+\frac{5}{8} = \frac{11}{8}$
	
	\item If less than $\frac{3}{4}$ is removed, then we can divide the removed bin into two groups, to one group add an item from each bin from the other group, and then pack each pair of items from the second group. 
\end{enumerate}


\comment{Put each item in $k$ in a single bin. Then, we find a packing using LP, since the number of fractional items is at most the size of the optimum, and they are all of size at most half, since items larger than 
}
\section{Perfect graph}
We improve the $2.5$ approximation of \cite{epstein2008bin} for perfect graphs. The algorithm described here relies on the following assumptions, and if they are incorrect, the algorithm may fail, thus we need to make sure that the following can indeed be solved with polynomial time. 

\begin{enumerate}
	\item There exists an algorithm that finds a maximum matching in perfect graph 
\end{enumerate}

Let the be an instance of Bin Packing with Perfect conflict graph (BPP) $\mathcal{I} = (I, (s_{\ell})_{\ell \in I},G = (I, E))$, where $I$ is the set of items, $s_{\ell}$ is the size of an item  $\ell \in I$ and $G$ is a perfect graph. Let $I = S \cup M \cup L$ where the {\em small} items are $S = \{\ell \in I | s_{\ell} \leq \frac{1}{3}\}$, the {\em medium} items are $M = \{\ell \in I |  \frac{1}{3} < s_{\ell} \leq \frac{1}{2}\}$, and the {\em large} items are $L = \{\ell \in I | s_{\ell} > \frac{1}{2}\}$. Denote the induced graph of a subset of vertices $X$ by $G[X]$. 


\begin{lemma}
	\label{lem:matching}
	There is an algorithm that finds the optimal packing of $J = (M\cup L, s_{\ell})_{\ell \in M\cup L}, G[M\cup L])$. 
\end{lemma}

\begin{proof}
	Maximum matching is the optimal solution, since there cannot be more than two items in the same bin without overflow. 
	\qed
\end{proof}


We split into two cases, depending on whether $s(S) \leq \frac{S(I)}{3}$ or not. First, recall the two lower bounds on the optimum. 

\begin{enumerate}
	\item $OPT \geq s(I)$. \label{1}
	
	\item $OPT \geq \chi(G)$.\label{2}
\end{enumerate}

\subsection{$s(S) \leq \frac{S(I)}{3}$}

By lemma~\ref{lem:matching} we can find an optimal packing of $J$ in at most $OPT(J) \leq OPT(\mathcal{I})$ bins. The algorithm find an optimal coloring of $G$. Each color $c$ with $s(c) \leq 1$ is a bin in our packing. The remaining color, can yield a bin which is $\frac{3}{4}$-full with residual. At the end, at most $\chi(G$ bins can be such that there are no more items to add, because each such bin is a full color of the graph. Moreover, each color which is with total size of items more than one, can construct a bin which is $\frac{3}{4}$-full, since the items are small.  The remaining items are in $S$, and can be packed in at most 

$$OPT+\chi(G)+\frac{4}{3} s(S) \leq OPT+ \chi(G)+\frac{4}{3} \frac{S(I)}{3} \leq 2+\frac{4}{9} OPT$$



\subsection{$s(S) > \frac{S(I)}{3}$}
In this case $s(M \cup L) < \frac{2S(I)}{3}$. Observe a maximum matching of $G[M\cup L]$. Each edge in the matching induce a bin with $\frac{2}{3}$ total size at least. The remaining unpaired item $\ell$ in $M \cup L$ have two options:

\begin{enumerate}
	\item If there are remaining items in $S$ that can be added to $\ell$ then this bin would be $\frac{3}{4}$-full. 
	
	\item If the3re are not enough items that can be added, then this bin is a color, as the remaining items cannot be packed with it, so there are no other representatives left from this color, and thus this color is removed.
\end{enumerate}

Overall, the number of bins used is 

$$\chi(G)+\frac{4}{3} s(S)+\frac{3}{2} s(M\cup L) \leq \chi(G)+\frac{4}{3} \frac{S(I)}{3}+\frac{3}{2} \frac{2S(I)}{3} \leq 2+\frac{4}{9} OPT$$


\section{General Bin Packing with Bipartite Conflict Graphs (BPB)}
The best known approximation ratio for this problem is $\frac{7}{4}$ by \cite{epstein2008bin}. A simple algorithm with improved approximation ratio is given below. Let $\mathcal{I} = (G(I = U \cup V, E), (s_i)_{i \in I})$ be a BPB instance, where $G$ is a bipartite graph and $s_i \in (0,1]$ is the size of item $i \in I$. Note that the sets of items $U,V$ form classic Bin packing instances. We assume that $OPT(\mathcal{I}) > 1$ throughout this section as the problem is trivial in this case and the problem can be solved optimally in polynomial time. 

\begin{lemma}
	\label{lem:asymptotic}
	For $OPT(\mathcal{I}) > 1$ it holds that $OPT(U)+OPT(V) \leq 1.5 OPT(\mathcal{I})+\frac{1}{2}$.
\end{lemma}

\begin{proof}
	Observe an optimal solution $OPT$ of $\mathcal{I}$ with $OPT(\mathcal{I}) = X > 1$ bins. Number the bins in this optimal solution (arbitrarily) $B_1, \ldots, B_X$. Let $B_i(U), B_i(V)$ be the items packed by $OPT$ in bin $B_i, i \in [X]$ from $U,V$, respectively. In addition, let $s(A)$ be the total size of items in $A \subseteq I$. 
	
	By the capacity constraint of the bins, it follows that  $s(B_i(U)) + s(B_i(V)) \leq 1$ and thus $s(B_i(U)) \leq \frac{1}{2}$ or $s(B_i(V)) \leq \frac{1}{2}$. Let $r(U), r(V)$ be the number of indices $i$ with respect to OPT, such that $s(B_i(U)) \leq \frac{1}{2}$, $s(B_i(V)) \leq \frac{1}{2}$, respectively. Formally, $r(U) = |\{i \in [X] | s(B_i(U)) \leq \frac{1}{2}\}|, r(V) = |\{i \in [X] | s(B_i(V)) \leq \frac{1}{2}\}|$. Moreover, let $R(U) = \{ B_i(U)| s(B_i(U)) \leq \frac{1}{2}\}, R(V) = \{B_i(V) | s(B_i(V)) \leq \frac{1}{2}\}$.
	
	it is proven below that
	\begin{equation}
		\label{eq:r>X}
		r(U)+r(V) \geq X
	\end{equation}
	
	Assume towards a contradiction that $r(U)+r(V) < X$. Therefore, there exists an index $i \in [X]$ such that $s(B_i(U)), s(B_i(V)) > \frac{1}{2}$. Contradiction that OPT is a feasible packing of $\mathcal{I}$. First, we assume that Inequality~\eqref{eq:r>X} is holding with equation, i.e., $r(U)+r(V) = X$. Otherwise, the claim is even easier to prove and the proof below also covers the case where $r(U)+r(V) > X$. There are several different cases for finishing the lemma, as follows. 
	
	\begin{enumerate}
		\item $X,|r(U)|,|r(V)| \in \mathbb{N}_{\text{even}}$. In this case, each pair $B_i(U), B_j(U), i \neq j \in [X], B_i(U), B_j(U) \in r(U)$ can be packed together, as there are no conflicts between items in $U$ and $s(B_i(U)) \leq \frac{1}{2}, s(B_j(U)) \leq \frac{1}{2}$. Similarly, the bins in $r(V)$ can be partitioned into pairs with similar attributes. It follows that the number of bins required for packing $U$ is at most:
		
		$$OPT(U) \leq \frac{r(U)}{2}+X-r(U) = X-\frac{r(U)}{2}$$
		
		Similarly, $OPT(V) \leq X-\frac{r(V)}{2}$. Hence, 
		
		$$OPT(U)+OPT(V) \leq X-\frac{r(U)}{2}+X-\frac{r(V)}{2} \leq 2X-\frac{X}{2} = 1.5X = 1.5 OPT(\mathcal{I})$$
		
		Where the last inequality is by~\ref{eq:r>X}.
		
		
		
		\item $X \in \mathbb{N}_{\text{even}}$,  $r(U), r(V) \in \mathbb{N}_{\text{odd}}$. Because $r(U), r(V) \in \mathbb{N}_{\text{odd}}$, all the bins except one in $U,V$ can be partitioned and packed in pairs. There must be $i \in [X]$ such that $B_i(U) \notin R(U)$ because $X \in \mathbb{N}_{\text{even}}$. Similarly, There must be $j \in [X]$ such that $B_j(V) \notin r(V)$. Because OPT is a feasible packing of $\mathcal{I}$, it follows that $s(B_i(U))+s(B_i(V)) \leq 1$, $s(B_j(U))+s(B_j(V)) \leq 1$. 
		
		Hence, $$s(B_i(U))+s(B_i(V))+s(B_j(U))+s(B_j(V)) \leq 2$$ then either $s(B_i(U))+s(B_j(U)) \leq 1$ or $s(B_j(U))+s(B_i(U)) \leq 1$ and assume w.l.o.g that $s(B_i(U))+s(B_j(U)) \leq 1$, and it follows that $B_j(U) \in R(U)$. 
		
		
		Therefore, $B_i(U)),B_j(U)$ can be packed in one bin, and the items in bins in $R(U) \setminus \{B_j(U)\}$ can be packed in at most $\frac{r(U)-1}{2}$ bins, since we can partition $R(U)$ into pairs, and pack each pair in one bin feasibly. In addition, the remaining items in $U$ (i.e., all items in $U$ that are in bins $k \in [X]$ in OPT for which $s(B_k(U)) > \frac{1}{2}$ excluding $B_i(U)$), can be packed in $X- R(U)-1$ bins, since these items are packed in $X- R(U)-1$ bins in OPT.
		
		Thus, overall
		
		\begin{equation}
			\label{eq:OPT(U)}
			OPT(U) \leq 1+\frac{r(U)-1}{2}+X-r(U)-1 = \frac{r(U)-1}{2}+X-r(U)
		\end{equation}
		Moreover, similarly to the previous case, the bins in $R(V)$ except for one bin can be partitioned into pairs and packed together and we get the following inequality: $OPT(V) \leq X-\frac{r(V)-1}{2}$.
		
		
		using the above inequalities and the previous case, the following holds. 
		
		$$OPT(U)+OPT(V) \leq \frac{r(U)-1}{2}+X-r(U)+X-\frac{r(V)-1}{2} \leq 2X-\frac{X}{2} = 1.5X = 1.5 OPT(\mathcal{I})$$
		
		
		
		
		
		\item $X \in \mathbb{N}_{\text{odd}}$ W.l.o.g $r(U) \in \mathbb{N}_{\text{even}}, r(V) \in \mathbb{N}_{\text{odd}}$. 
		Therefore, 
		
		$$OPT(U)+OPT(V) \leq \frac{r(U)}{2}+X-r(U)+\frac{r(V)-1}{2}+1+X-r(V) \leq 2X-\frac{X}{2}+\frac{1}{2} = $$
		$$1.5X+\frac{1}{2} = 1.5 OPT(\mathcal{I})+\frac{1}{2}$$
		
	\end{enumerate}
	\qed
\end{proof}



It follows that $U,V$ can be packed separately in two disjoint sets of bins using an algorithm for the classic Bin Packing problem. 



\begin{algorithm}[htb]
	\caption{NonConstantOptimum}
	\label{Alg:NonConstantOptimum}
	\begin{algorithmic}[1]
		\State{Pack $U$ using \cite{rothvoss2013approximating}}.
		\State{Pack $V$ using \cite{rothvoss2013approximating}}.
	\end{algorithmic}
\end{algorithm}

\begin{lemma}
	\label{lem:asymptotic2}
	There exists a constant $c$, such that for any instance $\mathcal{I}$ with $OPT(\mathcal{I}) > c$ it holds that Algorithm~\ref{Alg:NonConstantOptimum} returns a packing with at most $\frac{5}{3} OPT(\mathcal{I})$ bins.
\end{lemma}

\begin{proof}
	Using the approximation with additive approximation ratio of $O(log(OPT)loglog(OPT))$ \cite{rothvoss2013approximating}, the overall number of bins used in by Algorithm~\ref{Alg:NonConstantOptimum} is $$OPT(U)+O(log(OPT(U))loglog(OPT(U)))+OPT(V)+O(log(OPT(V))loglog(OPT(V)))$$
	
	By Lemma~\ref{lem:asymptotic} the number of bins is at most 
	
	$$1.5 OPT(\mathcal{I})+\frac{1}{2}+O(log(OPT(\mathcal{I}))loglog(OPT(\mathcal{I}))$$
	
	It can be easily seen that there is a constant $c$, such that $\frac{1}{2}+O(log(OPT(\mathcal{I}))loglog(OPT(\mathcal{I})) \leq (\frac{5}{3}-\frac{3}{2})OPT(\mathcal{I})$ for any $\mathcal{I}$ with $OPT(\mathcal{I}) > c$. The claim follows. 
	\qed
\end{proof}


\comment{
	This achieves a packing with at most  $1.5OPT(\mathcal{I})+\frac{1}{2}$ bins using Lemma~\ref{lem:asymptotic}. Note that for each instance $\mathcal{I}$ with $OPT(\mathcal{I}) \geq 3$ it holds that $1.5OPT(\mathcal{I})+\frac{1}{2} \leq \frac{5}{3} OPT(\mathcal{I})$ by simple arithmetic.} Thus, for instances where the optimum is larger than the  constant $c$ which exists by Lemma~\ref{lem:asymptotic2}, Algorithm~\ref{Alg:NonConstantOptimum} achieves $\frac{5}{3}$ approximation ratio. In addition, we provide an algorithm with $\frac{5}{3}$-approximation for the case where $OPT(\mathcal{I}) = O(1)$. Thus, overall achieving $\frac{5}{3}$-approximation for Bin Packing with Bipartite Conflicts graphs.

Th algorithm for $OPT(\mathcal{I}) = c = O(1)$ is given in the pseudocode of Algorithm~\ref{Alg:ConstantBins}. First, by the algorithm of $\frac{7}{4}$-approximation \cite{epstein2008bin} we can solve this problem with $3/2$ approximation for $c = 2,3$ bins. Thus, assume that $c \geq 4$. Let $\varepsilon =
\frac{1}{1000c}$. An item $i$ is {\em large} if $s_i > \varepsilon$, and the item is {\em tiny} otherwise. Let $T(U), T(V)$ be the set of tiny items in $U, V$, respectively, and let $L(U), L(V)$ be the set of tiny items in $U, V$, respectively. Denote by $s(A)$ the total size of items in $A \subseteq I$. 

The following is a definition of {\em packing}. Given a BPB instance $\mathcal{I} = (G(I = U \cup V, E), (s_i)_{i \in I})$, A packing of $S$ is a tuple $A = (A_1, \ldots, A_m)$ where $A_i \subseteq I, s(A_i) \leq 1, A_i \cap A_j = \emptyset, i, j \in [m]$ and for an edge $\{u,v\} \in E$ and $i \in [m]$ it holds that $|\{u,v\} \cap A_i| \leq 1$, and $S = A_1 \cup A_2 \cup \ldots \cup A_m$. The packing is {\em full} if $\cup_{i \in [m]} A_i = I$ and the packing is {\em partial} otherwise. Denote by $\#bins(A)$ the number of bins in the packing, i.e., $\#bins(A)=m$. 

Given a BPB instance $\mathcal{I} = (G(I = U \cup V, E), (s_i)_{i \in I})$ and a packing $A = (A_1, \ldots, A_m)$, ${\tilde A} =  ( {\tilde A}_1,  \ldots , {\tilde A}_m )$ is a {\em completion} of $A$ if $A^* = ( A_1 \cup {\tilde A}_1, \ldots, A_m \cup {\tilde A}_m
)$ is a full packing of $I$, such that ${\tilde A}_i \subseteq I \setminus (\cup_{j \in [m]} A_j), i \in [m]$. The algorithm handles differently instances, according to the following. Assume, w.l.o.g, that $s(L(V)) \geq s(L(U))$.  Let $Q = \argmax{}\: (s(T(U), s(T(V))), W = \argmin{}\: (s(T(U)), s(T(V)))$.

\comment{
	
	\begin{enumerate}
		\item if $s(L(V)) \leq \frac{c}{2}$.
		In this case the items in $L(U), L(V)$ are packed  optimally by enumeration in two disjoint sets of bins, and the tiny items are added ton these bins greedily, the items in $T(U)$ to the bins where $L(U)$ are packed, and $T(V)$ are added to the bins where the items in $L(V)$ are packed. Additional bins are added if necessary.
		
		\item if $s(L(V)) > \frac{c}{2}$. Then the items in $L(U), L(V)$ are packed by a packing which corresponds to the optimal packing of $\mathcal{I}$ (i.e., in at most $c$ bins). Then, the maximal argument (either $U$ or $V$) for $s(T(U)), s(T(V))$ is packed greedily in these at most $c$ bins. Additional bins are added for the remaining items in $T(U), T(V)$. 
	\end{enumerate}
}


\begin{algorithm}[htb]
	\caption{ConstantBins}
	\label{Alg:ConstantBins}
	\begin{algorithmic}[1]
		\If {$s(L(U) \cup T(U)) \leq 1$ or $s(L(V) \cup T(V)) \leq 1$}
		\If {$s(L(U) \cup T(U)) \leq 1$}
		\State{Pack $L(U) \cup T(U)$ in one bin and find a packing for $L(V) \cup T(V)$ in at most $c+1$ bins.}
		\Else 
		
		\State{Pack $L(V) \cup T(V)$ in one bin and find a packing for $L(U) \cup T(U)$ in at most $c+1$ bins.}
		\EndIf
		
		\Else
		\If {$OPT(L(V)) \leq \frac{c}{2}$}
		\State{Compute an optimal packing $P(L(V))$ for $L(V)$.} 
		\State{Compute an optimal packing $P(L(U))$ for $L(U)$.}
		\State{Add greedily, as many as possible feasibly, items from $T(U)$ to $P(L(U))$.}
		\State{Add greedily, as many as possible feasibly, items from $T(V)$ to $P(L(V))$.}
		\State{If there are unpacked items from $T(U)$}
		\Else 
		
		\State{Find a packing $R$ of $L(U)\cup L(V)$ in $c$ bins for which there is a completion of $\mathcal{I}$. }
		
		\State{Define the profit of an item to be equal to its size.}
		
		\State{Pack a maximum profit of items without conflicts in the bins using Multiple knapsack FPTAS for a constant number of bins.}
		
		\State{Let $Q'$ be the remaining items unpacked in $Q$.}
		
		\If {$c=4$}
		\If{$s(W) \leq 1$}
		\State{Pack $W, Q'$ each in one bin.}
		\Else 
		\State{Find a bin $b$ that can host the maximum profit of items from $W$ by removing items from $Q$ from this bin.}
		\State{Remove all items from $Q$ from the $c$ bins.}
		\State{Pack maximum profit of items from $Q$ in $b$}
		\State{Pack a maximum profit of items from $Q$ without conflicts in the remaining bins besides $b$}
		\State{Pack the remaining items from $W, Q$ each in one additional bin.}
		\EndIf
		\Else
		\State{Pack $W, Q'$ separately in additional bins.}
		\EndIf
		
		
		
		
		\State{Pack $L(V) \cup T(V)$ in one bin and find a packing for $L(U) \cup T(U)$ in at most $c+1$ bins.}
		
		\EndIf
		\EndIf
		
	\end{algorithmic}
\end{algorithm}









\begin{lemma}
	For $OPT(\mathcal{I}) = c > 2$ Algorithm~\ref{Alg:ConstantBins} returns a full packing of $\mathcal{I}$ in at most $\max(1.5 OPT(\mathcal{I}), OPT(\mathcal{I})+2)$ bins.
\end{lemma}

\begin{proof}
	We split the proof into several disjoint cases.
	
	\begin{enumerate}
		\item $s(L(U) \cup T(U)) \leq 1$ or $s(L(V) \cup T(V)) \leq 1$. Assume w.l.o.g that $s(L(U) \cup T(U)) \leq 1$. Then, because this is a bipartite graph, all items in $U$ can be packed in a single bin since there are no conflicts and there is no overflow. $V$ can be packed in $c+1$ bins by finding a packing of the large items in $V$ such that there exist a completion of this packing. Then, the items in $T(U)$ can be added using one additional bin, as each bin in the $c$ bin is full up to $1-\varepsilon$.  
		
		
		\item If $OPT(L(U)) \leq OPT(L(V)) \leq \frac{c}{2}$. We prove below that $s(L(V)) \geq \frac{\#P(L(V))}{2}$. Each two bins in $P(L(V))$ have total size of items strictly larger than $1$. The claim follows. Also, in this case we assume that $s(L(U) \cup T(U)) > 1$ and $s(L(V) \cup T(V)) > 1$. Thus, after filling greedily the tiny items in $P(L(V)), P(L(U))$, the total size of items packed is at least $(1-\varepsilon)\frac{c}{2}+1$. Hence, the total size left unpacked both from $Q, W$ is at most $\frac{c}{2}-1+\frac{\varepsilon c}{2}$. 
		
		\begin{enumerate}
			\item  If all of these items come either from $U$ or from $V$, then these items can be packed in additional $\frac{c}{2}$ bins, as we prove below. \begin{enumerate}
				\item If $\frac{c}{2} \in \mathbb{N}$, then because $\frac{\varepsilon c}{2} < \frac{1}{2}$ then items with total size $\frac{c}{2}-1+\frac{\varepsilon c}{2}$ and each item is with size smaller than $\varepsilon$, then these items can be packed in $\lceil \frac{c}{2}-1+\frac{\varepsilon c}{2} \rceil =  \frac{c}{2}$.
				
				\item Otherwise, $c$ is odd, and thus $OPT(L(U)) \leq OPT(L(V)) \leq \frac{c-1}{2}$. Therefore, we can pack the remaining items in $\frac{c+1}{2}$ bins, however, we use only $c-1$ bins at most in $P(L(V)), P(L(U))$ thus overall at most $1.5 c$ bins. 
			\end{enumerate}
			
			\item   Otherwise, it must be that both $P(L(V)), P(L(U))$ are filled with large and tiny items up to $1-\varepsilon$ in each bin, thus the total size left unpacked is at most $1$, and $2$ bins, one for $Q$ and one for $W$ are enough for a complete packing of $\mathcal{I}$ in $c+2$ bins. Overall, in this case at most $\max(1.5 OPT(\mathcal{I}), OPT(\mathcal{I})+2)$ bins. 
		\end{enumerate}
		
		
		
		
		
		
		
		
		\item  If $OPT(L(V))> \frac{c}{2}$. Then, by the algorithm, the $c$ bins in the packing obtained for $L(V)$ in this case contain items of total size at least $\frac{c}{4}$. 
		
		\begin{enumerate}
			\item If after the packing of $Q$ in these $c$ bins, there are no more items from $Q$ left unpacked, then $W$ can be packed in at most $\frac{c-\frac{c}{4}}{2}+1 = \lceil \frac{3c}{8}\rceil \leq \frac{3c}{8}+1$ bins. For $c \geq 8$ this is at most $\frac{c}{2}$ additional bins. For $c \leq 7$, it follows that $\frac{3c}{8} < \lceil \frac{3c}{8}\rceil-\varepsilon$, thus these items can be packed in $2$ bins for $c = 4,5$ and $3$ bins for $c = 6,7$, and thus at most $1.5 c $ bins overall. 
			
			
			
			\item Otherwise, if there are both items from $Q,W$ left unpacked, then:
			
			\begin{enumerate}
				\item For $c \geq 5$ then these items can be packed in at most $1+\lceil  \frac{3c}{8} \rceil \leq \frac{2c}{3}$ as in the previous case.
				
				\item If $c \leq 3$ then the algorithm of \cite{epstein2008bin} can be used with $3/2$-approximation for this particular case
				
				\item We now handle the case where $c = 4$. If $s(W) \leq 1$ then we can use $6$ overall. Otherwise, we choose one bin in the $4$ bins used for $L(U), L(V), Q$, remove the items from $Q$ from it and add the items from $W$, such that the remaining items from $W$, denoted by $W'$, are such that $s(W') \leq 1$. 
				
				Recall that $OPT(L(V))> \frac{c}{2} = 2$. Thus, $s(L(V)) > 1.5$ and thus $s(W)+s(Q) < 2.5 \rightarrow s(W) < 1.25$.  Assume that $s(W) = 1+d, d < 0.25$. Because $c = 4$, there exists a bin in the optimal packing of $\mathcal{I}$ that contains total size from $W$ at least $\frac{1+d}{4}$. In this optimal packing, there can be at most total size of $1-\frac{1+d}{4}$ items from $Q$. Thus, in the remaining three bins in this optimal solution, a total size of at least $s(Q)- (1-\frac{1+d}{4})$ can be packed. We can approximate this total size of packed items from $Q$ in this $3$ bins, and find a packing of items from $Q$ in this $3$ bins of total size at least $(1-\varepsilon) (s(Q)- (1-\frac{1+d}{4}))$. Moreover, we can find a packing of items from $W$ in the fourth bin (from which item from $Q$ where removed), of total size at least $(1-\varepsilon)\frac{1+d}{4}$. 
				
				The remaining items from $Q$ are of total size:
				
				$$s(Q) - (1-\varepsilon) (s(Q)- (1-\frac{1+d}{4})) = \varepsilon s(Q)-\frac{3}{4}\varepsilon+\frac{3}{4}-\frac{d}{4}+\frac{\varepsilon d}{4}$$
				
				It can be easily proven that for any $d < 0.25$ and for $\varepsilon < 0.01$ (for example..) these items can be packed in a single bin. 
				
				The remaining items from $W$ (i.e., $W'$) are of total size:
				
				$$1+d-(1-\varepsilon)\frac{1+d}{4} = \frac{3}{4}+\frac{3d}{4}+\frac{\varepsilon}{4}+\frac{\varepsilon d}{4}$$
				
				It can be easily proven that for any $d < 0.25$ and for $\varepsilon < 0.01$ (for example..) these items can be packed in a single bin. Overall $6$ bins. 
			\end{enumerate}
			
			
		\end{enumerate}
		
	\end{enumerate}
\end{proof}



\section{Sparse Bipartite Conflict Graphs}

In case that the number of edges is $\alpha n, \alpha = O(1)$, then we can construct an APTAS for this problem, explained shortly as follows. We note that there is a constant number of items which have more than $\alpha$ edges connected to them, and these items have their own labels for the enumeration. First, apply linear shifting for large items. Then, find using enumeration an (almost) optimal packing of the large items, and solve conflicts by swapping. Then, the small items can be added greedily, without creating conflicts. 

\section{APTAS for Complete Bipartite Conflict Graphs}
For the case where the bipartite is complete, it is easy to see that the optimum is to pack optimally each side of the bipartite. This can be done using an AFPTAS for classic Bin Packing. 
